House Price Modeling over Heterogeneous Regions with Hierarchical Spatial Functional Analysis

Online real-estate information systems such as Zillow and Trulia have gained increasing popularity in recent years. One important feature offered by these systems is the online home price estimate through automated data-intensive computation based on housing information and comparative market value analysis. State-of-the-art approaches model house prices as a combination of a latent land desirability surface and a regression from house features. However, by using uniformly damping kernels, they are unable to handle irregularly shaped regions or capture land value discontinuities within the same region due to the existence of implicit sub-communities, which are common in real-world scenarios. In this paper, we explore the novel application of recent advances in spatial functional analysis to house price modeling and propose the Hierarchical Spatial Functional Model (HSFM), which decomposes house values into land desirability at both the global scale and hidden local scales as well as the feature regression component. We propose statistical learning algorithms based on finite-element spatial functional analysis and spatial constrained clustering to train our model. Extensive evaluations based on housing data in a major Canadian city show that our proposed approach can reduce the mean relative house price estimation error down to 6.60%.

==> Makefile <==
DOCUMENT=main

default: clean $(DOCUMENT).pdf

$(DOCUMENT).pdf: $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex
	bibtex $(DOCUMENT)
	pdflatex $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex

all: $(DOCUMENT).pdf

clean:
	rm -rf *.aux $(DOCUMENT).log $(DOCUMENT).toc $(DOCUMENT).dvi \
    $(DOCUMENT).pdf $(DOCUMENT).bbl $(DOCUMENT).blg figs/*.fig.bak


==> backup.tex <==
Alternatives to the smoothing technique in \eqref{eq:min_err} exist, e.g., the thin plate spline penalty \cite{Sanga13} $\int_{\mathbb R^2}\big(\big(\frac{\partial^2 f}{\partial x^2}\big)^2+ 2 \big(\frac{\partial^2 f}{\partial x\partial y}\big)^2 + \big(\frac{\partial^2 f}{\partial y^2}\big)^2\big) \ud\mathbf p$ integrated over the entire plane and the soap film smoothing \cite{Wood08}.

It is shown in \cite{Sanga13} that the estimators $\hat{\boldsymbol{\beta}}$ and $\hat f$ that jointly solve problem \eqref{eq:min_err} exist unique. Specifically, for any function $h$ defined over $\Omega$, let $\mathbf h_n:=(h(\mathbf p_1),\ldots,h(\mathbf p_n))^{\mathsf T}$ denote the evaluations of the function $h$ on the $n$ training points. Then, $\hat{\boldsymbol{\beta}}$ and $\hat f$ are the ones that always satisfy
\begin{equation}\label{eq:cond_beta_f}
	\left\{
	\begin{array}{l}
\hat{\boldsymbol{\beta}} = (\mathbf W^{\mathsf T}\mathbf W)^{-1}\mathbf W^{\mathsf T}(\mathbf z-\hat{\mathbf f}_n)  \\
\mathbf u_n^{\mathsf T} \mathbf Q\hat{\mathbf f}_n + \lambda\int_{\Omega}\nabla^2 u\nabla^2 \hat f \ud\mathbf p = \mathbf u_n^{\mathsf T}\mathbf Q \mathbf z, 
	\end{array}
	\right.
\end{equation}
for any function $u$ % \where $H^2_{n0}(\Omega)$ be 
that meets certain smoothing and boundary conditions, 
%is \red{twice-differentiable} and has normal derivatives of $0$ on the boundary of $\Omega$
where $\mathbf Q = \mathbf I - \mathbf W(\mathbf W^{\mathsf T}\mathbf W)^{-1}\mathbf W^{\mathsf T}$.
This method can also be extended to guarantee that the surface $f$ have specific values at the boundary of the domain $\Omega$, or in some part of the boundary domain \cite{Sanga13}.


% Benefit of SSR:
Our approach will have the following advantages. 
%First, the feature vectors are split into the location and attributes information, with smoothed land value only depending on the location information. This gives a conceptually cleaner interpretation to the investment value of specific geographical regions.
\emph{First of all}, the above-mentioned spatial spline regression can handle the boundaries and holes (uninhabited areas) within a region of interest, such that the land values will drop to $0$ (or other desired values) at geographical boundaries. In contrast, as has been mentioned at the end of Sec. 2, the kernel-based methods will inevitably link different data artificially across areas where people cannot live, since the notion of ``neighbours'' solely depends on proximity and distances without considering holes between them and ill-shaped regions.
\emph{Second}, in kernel-based methods, the particular forms of kernel functions are hard to choose and the definition of neighbours is somehow artificial--- it is hard to know how close two properties need be in order to be counted as neighbours. In contrast, in finite element analysis, although we still need choose the form of piecewise polynomial functions for the triangles, yet as more fine-grained triangulation is applied when more data are available, approximation errors will vanish and the choice of specific piecewise polynomials becomes less critical. \emph{Last but not least}, the adapted finite element analysis turns the problem of solving \eqref{eq:cond_beta_f} into solving a system of linear equations. Using free or commercial finite element packages, it can be solved very efficiently, which further facilitates variable/feature selections for hedonic variables and other property attributes, increasing the power and efficiency of our model.


%In Case-Shiller (CS) repeat sales model \cite{Case89}, the \emph{log price} $p_{it}$ of property $i$ at time $t$ is modelled as $p_{it} = c_t + h_{it} + n_{it}$, where $c_t$ denotes the area wide price index, $h_{it}$ is a Gaussian random walk since the last sale of the house at time $t-1$, and $n_{it}$ is a random error. 
In this model, the error variance depends on the time interval between sales; changes in house values are likely to be more significant the longer the time between sales, %i.e., there is a drift in house prices over time. CS uses a three-stage least squares method to estimate the price index $c_t$. 
In fact, most traditional real-estate indices in use are based on this CS repeat sales methodology.
However, the simple hedonic and CS models are apparently insufficient to characterize complex spatio-temporal behavior of a large number of properties in the real-estate market.

